LQoCo: Learning to Optimize Cache Capacity Overloading in Storage Systems

Cache plays an important role to maintain high and stable performance (i.e. high throughput, low tail latency and throughput jitter) in storage systems. Existing rule-based cache management methods, coupled with engineers' manual configurations, cannot meet ever-growing requirements of both time-varying workloads and complex storage systems, leading to frequent cache overloading. In this paper, we for the first time propose a light-weight learning-based cache bandwidth control technique, called \LQoCo which can adaptively control the cache bandwidth so as to effectively prevent cache overloading in storage systems. Extensive experiments with various workloads on real systems show that LQoCo, with its strong adaptability and fast learning ability, can adapt to various workloads to effectively control cache bandwidth, thereby significantly improving the storage performance (e.g. increasing the throughput by 10\%-20\% and reducing the throughput jitter and tail latency by 2X-6X and 1.5X-4X, respectively, compared with two representative rule-based methods).

==> secs/Append.tex <==
% !TEX root = main.tex
\clearpage
\appendix
\section*{APPENDIX}
\label{appendix}
% \section{Architecture of commonly-used centralized storage system}
% \label{productionsystem}
% The architecture of the commonly-used centralized storage system is shown in Figure~\ref{OverallStructure}, with which our production-ready storage system is the same.
% \begin{figure}[h]
% \centering
% \includegraphics[width=3.3in]{./fig/OverallStructure.pdf}
% \caption{The commonly-used centralized storage system architecture (same with our production-ready platform) consists of a host-side system, caching tier and storage backend.}
% \label{OverallStructure}
% \end{figure}


\section{Example of Q table}
\label{appendix: q table}

Figure~\ref{qtable} shows an example of a Q table which is learned by the Q-learning algorithm in a period of 10 minutes. Each row of the table corresponds to one discretized state, of which column is the Q value for the corresponding discretized action. Note that the `invalid' in the table indicates that the corresponding action is forbidden to choose according to domain knowledge. Moreover, the states colored by red indicate extreme state while those colored by green indicate better states. For example, when the watermark level reaches High, the action of FastDecrease will be directly adopted. When the system is in a better state, the action of Keep is the only choice according to the value of entry of the table.

\begin{figure}[h]
\centering
\includegraphics[width=3.3in]{./fig/qtable.pdf}
\caption{An example of Q table. }
\label{qtable}
\end{figure}

\section{Evaluations for more intuition}
\label{intuitively}

\begin{figure}[!t]
\centering

\subfigure[Two cases (S-3 and S-4) in Linux platform. ]{
\includegraphics[width=3.3in]{./fig/linux_comparison.pdf}
}
\quad
\subfigure[Two cases (S-6 and S-14) in our production-ready platform. ]{
\includegraphics[width=3.3in]{./fig/twocases.pdf}
}
\caption{A set of cases on two platforms in Table~\ref{overallresult} for better visualizing the detailed comparison results. }
\label{fig:fourcases}
\end{figure}

The results of the four cases in two platforms are shown in Figure~\ref{fig:fourcases}. \LQoCo outperforms both \CoTo and `bypass' and the system without overload control methods.
\clearpage


\section{Pseudo code of Q-learning}
\label{appendix: alg}

Before describe the algorithm, several notations are supposed to be clarified:

1. $h_t = (S_{t-1}, A_{t-1}, R_t, S_t)$ represents one state transits to another state with action sampled from Q table.

2. $\mathcal{H}$ represents an experience buffer that stores the above transitions. The experience buffer will be updated periodically. Concretely, $N$ transition with top priorities will be kept within one update process.

3. For each transition $h_t\in \mathcal{H}$, $p_t$ denote its priority in the experience buffer.

4. $K$ represents the buffer update period.

5. $T$ denotes the Q table update period.

6. $k$ denotes the mini batch size.

7. $t$ represents the timer.

8. $\gamma$ denotes the discount factor.

9. $\eta$ denotes the learning rate.


10. $Q(S, A)$ denotes the Q table. The policy is drawn from the table with epsilon greedy strategy.

11. $\alpha$ represents how much prioritization is used.

12. $\beta$ is used to anneal the bias existing in prioritization.

\begin{algorithm}
\DontPrintSemicolon
  \KwInput{$\mathcal{H} = \{\}$, $t=0$, $p_1=1$ $K$, $N$, $k$, $\gamma$, $\alpha$, $\beta$}
%   \KwOutput{Your output}
%   \KwData{Testing set $x$}
    Initialize the policy $Q^{real}(,)$ and let $Q^{target}(,)=Q^{real}(,)$\\

    Observe $S_0$ and choose $A_0$ from $Q(S_0, *)$ with $\epsilon$-greedy strategy.

    \While{True}
    {
    Observe $S_t$ and calculate $R_t$ according to eq.(\ref{eq: reward1})\\
    Store transition $h_t = (S_{t-1}, A_{t-1}, R_t, S_t)$ into $\mathcal{H}$ with maximal priority $p_t=\max_{i<t} p_i$\\ \tcc{Here the new-added transition should have the maximal priority.}
    \If{$t \% K == 0$}
    {
        \tcp{Update the buffer}
        Keep $N$ transitions with top $N$ priorities from $\mathcal{H}$
    }
    \If{$t \% T == 0$}
    {
        \tcp{Update the Q table}
        \For{$j=1$ to $k$}
        {
          Sample transition $h_j \sim P(j)=\frac{p_j^\alpha}{\sum_{h_i \in \mathcal{H}} p_i^\alpha} $ from $\mathcal{H}$\\
          Compute importance-sampling weight $w_j=\frac{(N\times P(j))^{-\beta}}{max_i w_i}$\\
          Compute Temporal-Difference (TD) error:
          $\delta_j = R_j + \gamma Q^{target}(S_j, arg \max_a Q^{real}(S_j,a)) - Q^{real}(S_{j-1}, A_{j-1})$ \\
          Update priority of transition: $p_j=|\delta_j|$\\
          Update the value of Q table: $Q^{real}(S_{j-1}, A_{j-1})=Q^{real}(S_{j-1}, A_{j-1})+\eta \times w_j\times \delta_j$
        }
        \tcp{Periodically copy the value of real Q table to target Q table}
        Let $Q^{target}(,)=Q^{real}(,)$
    }
    Choose action $A_t$ from $Q^{real}(S_t, *)$ with $\epsilon$-greedy strategy\\
    t=t+1\\
    }
\caption{Prioritized Experience Replay for Online Q Learning}
\end{algorithm}

\section{Hyperparameter}
\label{appendix:hp}
Extensive experiments (grid searching) are conducted to perform hyperparameter selection. The recommended hyperparameters in \LQoCo framework are listed in Table~\ref{tab: hp-LQoCo}.

\begin{table}[h]
\caption{Hyperparameters in \LQoCo framework}
\label{tab: hp-LQoCo}
\scalebox{0.9}{
	\begin{tabular}{@{}cc@{}}
		\toprule
		Hyperparameter                 & Value/Range    \\
		\midrule
		% states
		watermark level: Extremely Low  &    [0, 10)      \\
		watermark level: Low           &    [10, 20)    \\
		watermark level: Mid           &    [30, 80)    \\
		watermark level: High          &    [80, 100]    \\

		processing ability: Low        &    (-1, -0.1]     \\
		processing ability: Mid        &    (-0.1, 0.1)   \\
		processing ability: High       &    [0.1, $+\infty$)   \\
		
		BDP: Low                       &    [0, 15)         \\
		BDP: Mid                       &    [15, 100)          \\
		BDP: High                      &    [100, $+\infty$)   \\
		
		% actions
		action: Fast Decrease	       &  -3\%     \\
		action: Slow Decrease	       &  -1\%     \\
		action: Slow Increase	       &  +1\%     \\
		action: Fast Increase	       &  +3\%     \\
		
		% reward weights
		weight of state watermark level ($f_W$) & 0.5   \\
        weight of processing ability ($f_P$) & 0.25     \\
        weight of BDP ($f_B$) & 0.25  \\

        probability of exploration ($\epsilon$) & 0.14  \\
	    \bottomrule
	\end{tabular}
	}
\end{table}



==> secs/abstract.tex <==
% !TEX root = main.tex

\begin{abstract}
%With the explosive growth of data, the storage systems are becoming larger and more complicated to meet the requirement of higher performance.

\textcolor{blue}{It is crucial for storage systems to maintain good and stable performance (such as high throughput and low tail latency) under varieties of workload. However, maintaining such performance within the storage system is extremely challenging. This is because the real-world workloads might be very time-varying. Besides, the architecture of current storage system is so complex and coupled that engineers are unable to directly find bottleneck and tune it. Empirically, we find that the optimization of cache overload might be a concise and effective solution to performance enhancement of the whole storage system. Nevertheless, few previous work about performance optimization of storage system pays attention on this problem.}

\textcolor{blue}{In this work, we propose a light-weight learning-based control framework called \LQoCo for solving cache overload problem in storage systems. To the best of our knowledge, it is the first work to solve this problem using reinforcement learning. Inside \LQoCo, a \textit{adaptive bound strategy} is elaborately designed to further improve the robustness and learning efficiency of the control framework. To verify the effectiveness of \LQoCo on improving performance of storage systems, extensive experiments in the Linux platform and the production-ready storage system~\footnote{One of the world's leading storage vendor which has provided professional storage services to over 12,000 enterprise-class customers in global.} under different workloads were performed. Compared with two rule-based overload control mechanisms, experimental results reveal that \LQoCo posses strong adaptability and fast learning ability, which significantly improves the overall performance of the storage system (such as higher throughput, lower tail latency and throughput jitter).}

% Maintaining sustainable high and stable performance under real-world workloads is a non-trivial work,
% especially for a cache which is the entry of the storage system which greatly affects the overall performance.
% Effective cache overload control mechanism for storage systems is crucial for protecting the system backend from overload. However, few studies focus on this problem. 


% \LQoCo using reinforcement learning which adopts the reward-feedback framework for bandwidth limiting. In addition, we design an effective reward function, useful domain knowledge and a safeguard bound strategy for \LQoCo to effectively improve the learning efficiency. We conduct extensive experiments in the Linux platform and the production-ready storage system~\footnote{One of the world's leading storage vendor which has provided professional storage services to over 12,000 enterprise-class customers in global.} under different workloads to demonstrate the superiority of \LQoCo. Experimental results show that \LQoCo has strong adaptability and significantly improves the performance with higher throughput, lower tail latency and throughput jitter compared to the baselines.  
\end{abstract}

